CP Violation in Top Physics

CP violation in top physics is reviewed. The Standard Model has negligible effects, consequently CP violation searches involving the top quark may constitute the best way to look for physics beyond the Standard Model. Non-standard sources of CP violation due to an extended Higgs sector with and without natural flavor conservation and supersymmetric theories are discussed. Experimental feasibility of detecting CP violation effects in top quark production and decays in high energy e+ e-, gamma-gamma, mu+ mu-, pp and p-bar p colliders are surveyed. Searches for the electric, electro-weak and the chromo-electric dipole moments of the top quark in e+ e- -> t-bar t and in p p -> t-bar t X are descibed. In addition, other mechanisms that appear promising for experiments, e.g., tree-level CP violation in e+ e- -> t-bar t h, t-bar t Z, t-bar t nu_e-bar nu_e and in the top decay t -> b tau nu_tau and CP violation driven by s-channel Higgs exchanges in p p, gamma gamma, mu+ mu- -> t-bar t etc., are also discussed.

==> titlepage/textabs.tex <==
CP violation in top physics is reviewed. The Standard Model has negligible
effects, consequently CP violation searches involving the top quark may
constitute the best way to look for physics beyond the Standard Model.
Non-standard sources of CP violation due to an extended Higgs sector with
and without natural flavor conservation and supersymmetric theories are
discussed. Experimental feasibility of detecting CP violation effects in
top quark production and decays in high energy e+ e-, gamma-gamma, mu+
mu-, pp and p-bar p colliders are surveyed.  Searches for the electric,
electro-weak and the chromo-electric dipole moments of the top quark in e+
e- -> t-bar t and in p p -> t-bar t X are descibed. In addition, other
mechanisms that appear promising for experiments, e.g., tree-level CP
violation in e+ e- -> t-bar t h, t-bar t Z, t-bar t nu_e-bar nu_e and in
the top decay t -> b tau nu_tau and CP violation driven by s-channel Higgs
exchanges in p p, gamma gamma, mu+ mu- -> t-bar t etc., are also
discussed. 



